Tackling Variabilities in Autonomous Driving

The state-of-the-art driving automation system demands extreme computational resources to meet rigorous accuracy and latency requirements. Though emerging driving automation computing platforms are based on ASIC to provide better performance and power guarantee, building such an accelerator-based computing platform for driving automation still present challenges. First, the workloads mix and performance requirements exposed to driving automation system present significant variability. Second, with more cameras/sensors integrated in a future fully autonomous driving vehicle, a heterogeneous multi-accelerator architecture substrate is needed that requires a design space exploration for a new form of parallelism. In this work, we aim to extensively explore the above system design challenges and these challenges motivate us to propose a comprehensive framework that synergistically handles the heterogeneous hardware accelerator design principles, system design criteria, and task scheduling mechanism. Specifically, we propose a novel heterogeneous multi-core AI accelerator (HMAI) to provide the hardware substrate for the driving automation tasks with variability. We also define system design criteria to better utilize hardware resources and achieve increased throughput while satisfying the performance and energy restrictions. Finally, we propose a deep reinforcement learning (RL)-based task scheduling mechanism FlexAI, to resolve task mapping issue. Experimental results show that with FlexAI scheduling, basically 100% tasks in each driving route can be processed by HMAI within their required period to ensure safety, and FlexAI can also maximally reduce the breaking distance up to 96% as compared to typical heuristics and guided random-search-based algorithms.

==> backup.tex <==
\begin{table}[h]
  \vspace{-1em} 
\scriptsize
\centering
\begin{tabular}{|p{0.7cm}<{\centering}|p{0.7cm}<{\centering}|p{0.9cm}<{\centering}|p{1cm}<{\centering}|p{1.2cm}<{\centering}|p{1.2cm}<{\centering}|}
\hline
 & \textbf{ISLPED\cite{ChenDi}} & \textbf{DE5-Net\cite{NaVi}} & \textbf{Eyeriss\cite{Eyeriss2}} & \textbf{YodaNN\cite{YodaNN}} & \textbf{P395-D8\cite{P395-D8}}  \\ \hline
AlexNet&30.6ms&45.7ms&\textgreater28.8ms&\textgreater54.73ms&20.1ms \\ \hline
VGG&151.8ms	&31.8ms&\textgreater1436.5ms&43.13 - 73.23ms&262.9ms\\ \hline
\end{tabular}
  \vspace{-1em} 
\caption{The latency for AlexNet and VGG in different hardware. \cite{Eyeriss2} and \cite{YodaNN} only counts convolutional layers, so the total latency for a entire network will be slightly larger than that given in their papers. At the same time, only the latency of VGG13 and VGG19 are given in \cite{YodaNN}. \label{ET}}
  \vspace{-1em} 
\end{table}


